Training-Free Mitigation of Language Reasoning Degradation After Multimodal Instruction Tuning

Multimodal models typically combine a powerful large language model (LLM) with a vision encoder and are then trained on multimodal data via instruction tuning. While this process adapts LLMs to multimodal settings, it remains unclear whether this adaptation compromises their original language reasoning capabilities. In this work, we explore the effects of multimodal instruction tuning on language reasoning performance. We focus on LLaVA, a leading multimodal framework that integrates LLMs such as Vicuna or Mistral with the CLIP vision encoder. We compare the performance of the original LLMs with their multimodal-adapted counterparts across eight language reasoning tasks. Our experiments yield several key insights. First, the impact of multimodal learning varies between Vicuna and Mistral: we observe a degradation in language reasoning for Mistral but improvements for Vicuna across most tasks. Second, while multimodal instruction learning consistently degrades performance on mathematical reasoning tasks (e.g., GSM8K), it enhances performance on commonsense reasoning tasks (e.g., CommonsenseQA). Finally, we demonstrate that a training-free model merging technique can effectively mitigate the language reasoning degradation observed in multimodal-adapted Mistral and even improve performance on visual tasks.

==> tables/open_source_instruction_data.tex <==
\begin{table*}[t]
    \centering 
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth} p{0.1\linewidth}p{0.2\linewidth}p{0.2\linewidth} }
        \toprule
          \textbf{Dataset Name} & \textbf{Link} & \textbf{Size}  & \textbf{How to Created} & \textbf{Tasks}  \\
        \toprule
        Dolly~\citeyear{conover2023free} & databricks/databricks-dolly-15k & 15K & Human Annotation & Creative Writing, Closed QA, Open QA, Summarization, Information Extraction, Classification, Brainstorming\\
        \midrule
        Alpaca & \url{https://github.com/tatsu-lab/stanford_alpaca?tab=readme-ov-file#data-release} & 55K & Self-Instruct type of synthetic generated data by GPT-3 & Each instance is for different tasks. \\
        \midrule
        MOSS~\citeyear{sun2024moss} & \url{https://github.com/OpenMOSS/MOSS/tree/main/SFT_data} & 1100K & GPT-3 generated & Brainstorming, Complex Instruction, Code, Role Playing, Writing, Harmless and Others. \\
        \midrule
        Alpaca-CoT~\citeyear{alpacacot2023} & QingyiSi/Alpaca-CoT & - & Mix & Mix of Instruction fine-tuning data\\ 
        

    \bottomrule
    \end{tabular}
    % }
    \caption{A List of Open Source Instruction Following Data}
    \label{tab:instruction_data}
\end{table*}

